DIAMOND: Taming Sample and Communication Complexities in Decentralized Bilevel Optimization

Decentralized bilevel optimization has received increasing attention recently due to its foundational role in many emerging multi-agent learning paradigms (e.g., multi-agent meta-learning and multi-agent reinforcement learning) over peer-to-peer edge networks. However, to work with the limited computation and communication capabilities of edge networks, a major challenge in developing decentralized bilevel optimization techniques is to lower sample and communication complexities. This motivates us to develop a new decentralized bilevel optimization called DIAMOND (decentralized single-timescale stochastic approximation with momentum and gradient-tracking). The contributions of this paper are as follows: i) our DIAMOND algorithm adopts a single-loop structure rather than following the natural double-loop structure of bilevel optimization, which offers low computation and implementation complexity; ii) compared to existing approaches, the DIAMOND algorithm does not require any full gradient evaluations, which further reduces both sample and computational complexities; iii) through a careful integration of momentum information and gradient tracking techniques, we show that the DIAMOND algorithm enjoys $\mathcal{O}(\epsilon^{-3/2})$ in sample and communication complexities for achieving an $\epsilon$-stationary solution, both of which are independent of the dataset sizes and significantly outperform existing works. Extensive experiments also verify our theoretical findings.

==> Sec1_Introduction.tex <==
% !TEX root = main.tex

% ----------------------- %
% Finished %
% ----------------------- %

\section{Introduction} \label{sec: Introduction}
Machine learning has been applied more frequently to edge networks, and the training phases of machine learning can be mathematically formulated as solving optimization problems. 
This brings attention to decentralized bilevel optimization in the networking and machine learning communities because of its ability to support many decentralized learning paradigms on peer-to-peer networks (e.g., multi-agent meta-learning~\cite{liu2021boml, rajeswaran2019meta}, multi-agent hyperparameter optimization~\cite{mackay2019self, okuno2021lp}, and multi-agent reinforcement learning~\cite{hong2020two, zhang2020bi}).

Decentralized bilevel optimization models the hierarchically structured problems, where the variables in the upper-level subproblems depend on the optimized variables in the lower-level subproblems~\cite{dempe2002foundations}. 
Single-agent bilevel optimization shares the same model as decentralized bilevel optimization, and it receives increasing attention due to the non-convexity in these problems. 
Inspired by the efficiency of gradient descent in machine learning, a natural method to deal with bilevel optimization problems is to alternate stochastic gradient descent (SGD) over upper- and lower-level subproblems.
Since only the approximation of the lower-level minimizer is used in the upper-level subproblem, the stochastic hypergradient of the upper-level subproblem is calculated in a biased way~\cite{khanduri2021near}.
To improve the accuracy of the upper-level hypergradient estimation, two approaches have been considered: 1) applying double-loop algorithms~\cite{ghadimi2018approximation, ji2021bilevel, yang2021provably}, and 2) applying single-loop algorithms~\cite{chen2021single, guo2021randomized, hong2020two, khanduri2021near}.
The double-loop algorithms take multiple inner-iterations and are more nature to consider.
However, the sample complexity for solving the lower-level optimization subproblem may be high.
On the other side, the single-loop algorithms iteratively solve the upper- and lower-level subproblems and update corresponding parameters simultaneously.
They are easier to implement and have higher computation efficiency.

Compared to single-agent bilevel optimization, which has only one optimization task in the lower-level subproblem, decentralized bilevel optimization needs to treat multiple lower-level tasks of different agents. 
Therefore, it is challenging to apply techniques designed for single-agent bilevel optimization to decentralized bilevel optimization due to the efficiency and scalability.
In addition, although decentralized optimization has been widely studied in recent years~\cite{lian2017can, sun2020improving, xin2021hybrid, zhang2021low}, the algorithmic ideas of it cannot be directly extended to decentralized bilevel optimization because of two reasons: 1) they focus on single-level optimization problems, and 2) the stochastic gradient estimators they used are unbiased, while the stochastic hypergradient of the upper-level subproblem for decentralized bilevel optimization is biased.
Besides, the coupled structure of the decentralized bilevel optimization problems and the non-convexity of these problems make it challenging to design algorithms and theoretically analyze their performance.

In decentralized bilevel optimization settings, multiple agents distributively solve the lower-level tasks locally and collaboratively optimize the global task through the peer-to-peer communication networks. 
It is nature to utilize decentralized network-consensus optimization methods~\cite{yau2022docom, zhang2021gt} to decentralized bilevel optimization.
In decentralized network-consensus optimization, a group of geographically dispersed computing nodes cooperate to solve an optimization problem.
Each node is associated with a local dataset that could not be aggregated due to the communication cost or the privacy/security concerns.
Thus, they need to exchange information with their neighbors to reach a consensus on the global optimal solution.

However, the design of network-consensus methods for decentralized bilevel optimization has two fundamental challenges that are conflict: 
1) The quality of the stochastic gradient estimator depends heavily on the number of samples used.
However, more samples lead to higher computational cost, and the computing resource in edge-computing environments is limited.
2) The intention to reduce the computational cost by using fewer samples per iteration would make the stochastic gradient more inaccurate. 
This would slow down the convergence and require more communication rounds to achieve a certain training accuracy.
Poor communication efficiency is especially problematic in wireless edge networks, since the communication links could be low-speed and highly dynamic.

To date, the existing decentralized bilevel optimization algorithms, which are INTERACT and SVR-INTERACT~\cite{Liu2022interact}, only have low communication complexity but high sample complexity (see more details in Section~\ref{sec: RelatedWork}). This limitation prompts the following question: \textit{How to design a decentralized bilevel optimization algorithm that achieves a good balance between sample complexity and communication complexity?}

To overcome the aforementioned challenges and achieve both low sample and communication complexities, we propose a new algorithm called \alg for decentralized bilevel optimization. 
Our main contributions are summarized as follows:
\begin{itemize}
    \item We propose a new algorithm named \alg (\ul{d}ecentralized s\ul{i}ngle-timescale stoch\ul{a}stic approxi\ul{m}ation with m\ul{o}me\ul{n}tum and gra\ul{d}ient-tracking) for solving stochastic bilevel optimization problems on decentralized multi-agent settings over networks. 
    \alg relies on network-consensus updates along with gradient tracking and uses a momentum-based stochastic gradient estimator, which reduces both sample and computational complexities.
    In addition, \alg uses a single-timescale structure, which reduces the computational cost and is easier to implement.
    
    \item We theoretically show that the \alg algorithm achieves the sample complexity of $\mathcal{O}(\epsilon^{-3/2})$ to find an $\epsilon$-stationary solution for non-convex upper-level optimization objectives, which matches the optimal sample complexity of SGD-type algorithms for solving single-level stochastic gradient problems. 
    Meanwhile, the communication complexity of \alg is $\mathcal{O}(\epsilon^{-3/2})$.
    These results demonstrate that our \alg strikes a good balance between sample and communication complexities.
    
    \item To validate the theoretical results of the proposed \alg algorithm, we conduct numerical experiments on a meta-learning problem using MNIST dataset. The numerical results show that \alg outperforms other SGD-based baseline algorithms in terms of sample complexities in various communication network settings.
   
\end{itemize}

The rest of the paper is organized as follows. 
Related work is given in Section~\ref{sec: RelatedWork}.
Section~\ref{sec: Preliminary} introduces the preliminaries, which are the peer-to-peer network model and the decentralized bilevel optimization problem. 
Section~\ref{sec: Algorithm} proposes the \alg algorithm, and the theoretical analysis of the convergence of \alg is presented in Section~\ref{sec: ConvergenceAnalysis}. 
Numerical results are reported in Section~\ref{sec: NumericalResults} to support our theoretical findings.
Section~\ref{sec: Conclusion} gives a conclusion of this paper.
